A Multi-Agent Perspective on Modern Information Retrieval

The rise of large language models (LLMs) has introduced a new era in information retrieval (IR), where queries and documents that were once assumed to be generated exclusively by humans can now also be created by automated agents. These agents can formulate queries, generate documents, and perform ranking. This shift challenges some long-standing IR paradigms and calls for a reassessment of both theoretical frameworks and practical methodologies. We advocate for a multi-agent perspective to better capture the complex interactions between query agents, document agents, and ranker agents. Through empirical exploration of various multi-agent retrieval settings, we reveal the significant impact of these interactions on system performance. Our findings underscore the need to revisit classical IR paradigms and develop new frameworks for more effective modeling and evaluation of modern retrieval systems.

==> abstract.tex <==
For decades, IR systems operated under the assumption that humans are
both the creators of content and the ones searching for it.
With the rise of
LLMs, this assumption does not hold anymore.
LLMs now actively participate in query formulation, document
generation, and ranking. We argue that the resultant emerging multi-agent
retrieval setting, composed of query, document and ranker agents,
calls for special consideration. For example, some
classical retrieval paradigms and principles fall short and should be
re-considered. 
We then discuss the different agents (query, document and ranker) and their interplay.
In addition, we
present empirical exploration performed with various multi-agent
retrieval settings. Analysis reveals the significant effects of the connections between the types of agents employed to generate queries and documents and those used to induce rankings.

==> experiments/online/evaluation.tex <==

The effectiveness of \botagents is measured by their average rank.

